A Systematic Comparison of Syntactic Representations of Dependency Parsing

We compare the performance of a transition-based parser in regards to different annotation schemes. We pro-pose to convert some specific syntactic constructions observed in the universal dependency treebanks into a so-called more standard representation and to evaluate parsing performances over all the languages of the project. We show that the ``standard'' constructions do not lead systematically to better parsing performance and that the scores vary considerably according to the languages.

==> res.tex <==
\begin{supertabular}{llrrr}
\toprule
   &      & transformed &     ud &                      diff \\
lang & transfo &             &        &                           \\
ar & case &      74.05\% & 73.36\% & \textcolor{green}{-0.70\%} \\
   & conjunction &      72.35\% & 75.83\% &    \textcolor{red}{3.49\%} \\
   & copule &      74.19\% & 73.85\% & \textcolor{green}{-0.35\%} \\
   & det &      73.36\% & 73.63\% &    \textcolor{red}{0.27\%} \\
   & mark &      73.68\% & 73.65\% &                    -0.02\% \\
   & mwe &      73.64\% & 73.62\% &                    -0.02\% \\
bg & case &      75.16\% & 75.95\% &    \textcolor{red}{0.79\%} \\
   & conjunction &      75.85\% & 76.88\% &    \textcolor{red}{1.03\%} \\
   & copule &      76.60\% & 76.69\% &                     0.09\% \\
   & det &      75.92\% & 75.88\% &                    -0.05\% \\
   & mark &      75.79\% & 76.07\% &    \textcolor{red}{0.28\%} \\
   & mwe &      76.25\% & 75.89\% & \textcolor{green}{-0.37\%} \\
   & name &      75.95\% & 75.96\% &                     0.01\% \\
ca & case &      80.36\% & 80.50\% &    \textcolor{red}{0.14\%} \\
   & conjunction &      79.86\% & 81.00\% &    \textcolor{red}{1.15\%} \\
   & copule &      81.02\% & 80.79\% & \textcolor{green}{-0.24\%} \\
   & det &      80.20\% & 80.59\% &    \textcolor{red}{0.39\%} \\
   & mark &      79.72\% & 80.32\% &    \textcolor{red}{0.60\%} \\
   & mwe &      80.43\% & 80.42\% &                    -0.01\% \\
   & name &      80.55\% & 80.45\% &                    -0.09\% \\
cu & case &      83.79\% & 83.05\% & \textcolor{green}{-0.74\%} \\
   & conjunction &      83.09\% & 83.25\% &    \textcolor{red}{0.15\%} \\
   & det &      83.27\% & 83.66\% &    \textcolor{red}{0.39\%} \\
   & mark &      83.08\% & 83.28\% &    \textcolor{red}{0.21\%} \\
da & case &      70.37\% & 70.35\% &                    -0.03\% \\
   & conjunction &      72.50\% & 73.05\% &    \textcolor{red}{0.55\%} \\
   & copule &      71.51\% & 71.75\% &    \textcolor{red}{0.23\%} \\
   & det &      70.51\% & 70.62\% &    \textcolor{red}{0.11\%} \\
   & mark &      70.24\% & 71.22\% &    \textcolor{red}{0.98\%} \\
   & mwe &      71.02\% & 71.13\% &    \textcolor{red}{0.11\%} \\
de & case &      72.68\% & 72.24\% & \textcolor{green}{-0.44\%} \\
   & conjunction &      72.57\% & 72.50\% &                    -0.07\% \\
   & copule &      72.78\% & 72.14\% & \textcolor{green}{-0.64\%} \\
   & det &      71.60\% & 71.72\% &    \textcolor{red}{0.12\%} \\
   & mark &      71.86\% & 72.02\% &    \textcolor{red}{0.16\%} \\
   & name &      72.15\% & 72.31\% &    \textcolor{red}{0.16\%} \\
el & case &      74.13\% & 73.50\% & \textcolor{green}{-0.63\%} \\
   & conjunction &      72.81\% & 73.77\% &    \textcolor{red}{0.95\%} \\
   & copule &      75.22\% & 73.87\% & \textcolor{green}{-1.35\%} \\
   & det &      73.13\% & 73.55\% &    \textcolor{red}{0.42\%} \\
   & mark &      72.90\% & 73.77\% &    \textcolor{red}{0.87\%} \\
en & case &      75.79\% & 75.59\% & \textcolor{green}{-0.20\%} \\
   & conjunction &      75.54\% & 76.23\% &    \textcolor{red}{0.68\%} \\
   & copule &      76.00\% & 76.05\% &                     0.05\% \\
   & det &      75.56\% & 75.61\% &                     0.05\% \\
   & mark &      75.72\% & 75.73\% &                     0.01\% \\
   & mwe &      75.62\% & 75.73\% &    \textcolor{red}{0.11\%} \\
   & name &      75.42\% & 75.73\% &    \textcolor{red}{0.31\%} \\
es & case &      76.78\% & 76.37\% & \textcolor{green}{-0.41\%} \\
   & conjunction &      74.66\% & 76.76\% &    \textcolor{red}{2.10\%} \\
   & copule &      77.47\% & 76.82\% & \textcolor{green}{-0.65\%} \\
   & det &      74.91\% & 75.79\% &    \textcolor{red}{0.88\%} \\
   & mark &      76.01\% & 75.83\% & \textcolor{green}{-0.18\%} \\
   & mwe &      76.19\% & 75.91\% & \textcolor{green}{-0.28\%} \\
   & name &      75.96\% & 75.85\% & \textcolor{green}{-0.10\%} \\
et & case &      66.89\% & 67.32\% &    \textcolor{red}{0.43\%} \\
   & conjunction &      66.37\% & 67.33\% &    \textcolor{red}{0.96\%} \\
   & copule &      70.38\% & 67.95\% & \textcolor{green}{-2.42\%} \\
   & det &      67.04\% & 67.53\% &    \textcolor{red}{0.49\%} \\
   & name &      66.99\% & 66.96\% &                    -0.03\% \\
eu & case &      66.00\% & 65.77\% & \textcolor{green}{-0.23\%} \\
   & conjunction &      66.56\% & 66.53\% &                    -0.03\% \\
   & copule &      68.23\% & 67.42\% & \textcolor{green}{-0.81\%} \\
   & det &      64.49\% & 65.52\% &    \textcolor{red}{1.03\%} \\
   & mark &      65.78\% & 65.95\% &    \textcolor{red}{0.18\%} \\
   & mwe &      66.14\% & 66.20\% &                     0.06\% \\
   & name &      66.04\% & 65.84\% & \textcolor{green}{-0.20\%} \\
fa & case &      75.47\% & 74.58\% & \textcolor{green}{-0.89\%} \\
   & conjunction &      74.14\% & 75.61\% &    \textcolor{red}{1.48\%} \\
   & copule &      78.13\% & 78.08\% &                    -0.05\% \\
   & det &      74.72\% & 74.54\% & \textcolor{green}{-0.18\%} \\
   & mark &      75.44\% & 74.75\% & \textcolor{green}{-0.68\%} \\
   & name &      74.69\% & 74.70\% &                     0.01\% \\
fi & case &      64.35\% & 63.80\% & \textcolor{green}{-0.55\%} \\
   & conjunction &      63.51\% & 64.99\% &    \textcolor{red}{1.47\%} \\
   & copule &      66.59\% & 64.30\% & \textcolor{green}{-2.30\%} \\
   & mark &      64.36\% & 63.97\% & \textcolor{green}{-0.40\%} \\
   & mwe &      63.84\% & 63.97\% &    \textcolor{red}{0.13\%} \\
   & name &      64.18\% & 63.85\% & \textcolor{green}{-0.33\%} \\
fr & case &      74.66\% & 74.91\% &    \textcolor{red}{0.25\%} \\
   & conjunction &      73.87\% & 74.55\% &    \textcolor{red}{0.68\%} \\
   & copule &      75.29\% & 74.61\% & \textcolor{green}{-0.69\%} \\
   & det &      73.21\% & 74.74\% &    \textcolor{red}{1.53\%} \\
   & mark &      74.53\% & 74.57\% &                     0.04\% \\
   & mwe &      74.66\% & 74.41\% & \textcolor{green}{-0.25\%} \\
   & name &      74.84\% & 74.58\% & \textcolor{green}{-0.25\%} \\
ga & case &      70.61\% & 69.90\% & \textcolor{green}{-0.71\%} \\
   & conjunction &      68.06\% & 70.03\% &    \textcolor{red}{1.97\%} \\
   & copule &      70.17\% & 70.01\% & \textcolor{green}{-0.17\%} \\
   & det &      68.64\% & 68.50\% & \textcolor{green}{-0.13\%} \\
   & mark &      69.41\% & 68.42\% & \textcolor{green}{-0.99\%} \\
   & name &      69.79\% & 69.46\% & \textcolor{green}{-0.33\%} \\
gl & case &      72.17\% & 77.21\% &    \textcolor{red}{5.04\%} \\
   & conjunction &      76.76\% & 77.24\% &    \textcolor{red}{0.48\%} \\
   & copule &      77.37\% & 77.15\% & \textcolor{green}{-0.23\%} \\
   & det &      76.36\% & 77.39\% &    \textcolor{red}{1.03\%} \\
   & mark &      77.14\% & 77.36\% &    \textcolor{red}{0.22\%} \\
got & case &      82.04\% & 80.89\% & \textcolor{green}{-1.15\%} \\
   & conjunction &      80.17\% & 81.17\% &    \textcolor{red}{1.00\%} \\
   & det &      81.08\% & 81.53\% &    \textcolor{red}{0.45\%} \\
   & mark &      80.92\% & 81.46\% &    \textcolor{red}{0.54\%} \\
grc & case &      59.92\% & 58.80\% & \textcolor{green}{-1.12\%} \\
   & conjunction &      59.21\% & 59.92\% &    \textcolor{red}{0.71\%} \\
   & copule &      60.22\% & 60.34\% &    \textcolor{red}{0.12\%} \\
   & det &      60.87\% & 59.37\% & \textcolor{green}{-1.49\%} \\
   & mark &      59.41\% & 58.65\% & \textcolor{green}{-0.76\%} \\
he & case &      74.67\% & 75.91\% &    \textcolor{red}{1.24\%} \\
   & conjunction &      74.80\% & 77.15\% &    \textcolor{red}{2.35\%} \\
   & copule &      75.99\% & 75.97\% &                    -0.02\% \\
   & det &      75.74\% & 75.63\% & \textcolor{green}{-0.11\%} \\
   & mark &      75.80\% & 75.84\% &                     0.04\% \\
   & mwe &      75.96\% & 76.14\% &    \textcolor{red}{0.18\%} \\
   & name &      76.34\% & 76.24\% &                    -0.10\% \\
hi & case &      86.11\% & 86.77\% &    \textcolor{red}{0.66\%} \\
   & conjunction &      87.04\% & 87.49\% &    \textcolor{red}{0.45\%} \\
   & det &      86.49\% & 86.75\% &    \textcolor{red}{0.26\%} \\
   & mark &      86.83\% & 86.79\% &                    -0.04\% \\
hr & case &      68.37\% & 69.56\% &    \textcolor{red}{1.19\%} \\
   & conjunction &      69.26\% & 70.71\% &    \textcolor{red}{1.46\%} \\
   & copule &      69.20\% & 70.02\% &    \textcolor{red}{0.82\%} \\
   & det &      67.99\% & 69.59\% &    \textcolor{red}{1.60\%} \\
   & mark &      69.59\% & 69.45\% & \textcolor{green}{-0.15\%} \\
   & mwe &      69.36\% & 69.91\% &    \textcolor{red}{0.55\%} \\
   & name &      69.47\% & 69.10\% & \textcolor{green}{-0.38\%} \\
hu & case &      70.46\% & 70.19\% & \textcolor{green}{-0.28\%} \\
   & conjunction &      70.19\% & 70.99\% &    \textcolor{red}{0.80\%} \\
   & copule &      70.76\% & 70.15\% & \textcolor{green}{-0.60\%} \\
   & det &      68.68\% & 70.39\% &    \textcolor{red}{1.71\%} \\
   & mark &      70.50\% & 69.75\% & \textcolor{green}{-0.75\%} \\
id & case &      72.43\% & 72.45\% &                     0.02\% \\
   & conjunction &      72.23\% & 73.55\% &    \textcolor{red}{1.33\%} \\
   & copule &      72.54\% & 72.49\% &                    -0.06\% \\
   & det &      71.55\% & 71.76\% &    \textcolor{red}{0.21\%} \\
   & mark &      72.49\% & 72.13\% & \textcolor{green}{-0.35\%} \\
   & name &      72.43\% & 72.50\% &                     0.08\% \\
it & case &      79.81\% & 79.43\% & \textcolor{green}{-0.39\%} \\
   & conjunction &      79.85\% & 80.23\% &    \textcolor{red}{0.38\%} \\
   & copule &      78.26\% & 79.45\% &    \textcolor{red}{1.19\%} \\
   & det &      78.92\% & 79.51\% &    \textcolor{red}{0.59\%} \\
   & mark &      79.68\% & 79.54\% & \textcolor{green}{-0.14\%} \\
   & mwe &      79.37\% & 79.47\% &                     0.10\% \\
   & name &      79.59\% & 79.37\% & \textcolor{green}{-0.22\%} \\
kk & case &      56.62\% & 59.67\% &    \textcolor{red}{3.05\%} \\
   & conjunction &      61.52\% & 61.76\% &    \textcolor{red}{0.25\%} \\
   & det &      57.23\% & 58.25\% &    \textcolor{red}{1.02\%} \\
   & mark &      57.43\% & 57.23\% & \textcolor{green}{-0.20\%} \\
   & name &      58.45\% & 59.47\% &    \textcolor{red}{1.02\%} \\
la & case &      59.98\% & 58.75\% & \textcolor{green}{-1.24\%} \\
   & conjunction &      52.57\% & 60.69\% &    \textcolor{red}{8.11\%} \\
   & copule &      59.34\% & 56.47\% & \textcolor{green}{-2.87\%} \\
   & mark &      58.88\% & 58.99\% &    \textcolor{red}{0.11\%} \\
lv & case &      52.08\% & 52.21\% &    \textcolor{red}{0.13\%} \\
   & conjunction &      51.94\% & 52.40\% &    \textcolor{red}{0.47\%} \\
   & det &      52.51\% & 52.64\% &    \textcolor{red}{0.13\%} \\
   & mark &      53.50\% & 52.28\% & \textcolor{green}{-1.22\%} \\
   & mwe &      53.66\% & 54.12\% &    \textcolor{red}{0.46\%} \\
   & name &      52.67\% & 52.87\% &    \textcolor{red}{0.20\%} \\
nl & case &      66.11\% & 66.95\% &    \textcolor{red}{0.84\%} \\
   & conjunction &      70.51\% & 70.09\% & \textcolor{green}{-0.42\%} \\
   & copule &      69.82\% & 67.73\% & \textcolor{green}{-2.09\%} \\
   & det &      67.84\% & 66.86\% & \textcolor{green}{-0.99\%} \\
   & mark &      67.45\% & 67.66\% &    \textcolor{red}{0.21\%} \\
   & name &      67.15\% & 67.33\% &    \textcolor{red}{0.18\%} \\
no & case &      77.59\% & 78.36\% &    \textcolor{red}{0.76\%} \\
   & conjunction &      77.64\% & 78.45\% &    \textcolor{red}{0.81\%} \\
   & copule &      79.68\% & 78.42\% & \textcolor{green}{-1.26\%} \\
   & det &      78.08\% & 78.15\% &                     0.07\% \\
   & mark &      77.66\% & 78.23\% &    \textcolor{red}{0.57\%} \\
   & name &      78.29\% & 78.44\% &    \textcolor{red}{0.15\%} \\
pl & case &      72.67\% & 72.81\% &    \textcolor{red}{0.14\%} \\
   & conjunction &      72.25\% & 72.77\% &    \textcolor{red}{0.52\%} \\
   & copule &      74.71\% & 73.40\% & \textcolor{green}{-1.31\%} \\
   & det &      72.59\% & 72.96\% &    \textcolor{red}{0.38\%} \\
   & mark &      72.60\% & 72.87\% &    \textcolor{red}{0.27\%} \\
pt & case &      73.40\% & 73.37\% &                    -0.02\% \\
   & conjunction &      73.46\% & 74.38\% &    \textcolor{red}{0.92\%} \\
   & copule &      74.90\% & 73.77\% & \textcolor{green}{-1.13\%} \\
   & det &      73.48\% & 73.82\% &    \textcolor{red}{0.34\%} \\
   & mwe &      73.78\% & 73.11\% & \textcolor{green}{-0.67\%} \\
   & name &      74.09\% & 73.73\% & \textcolor{green}{-0.36\%} \\
ro & case &      72.06\% & 71.69\% & \textcolor{green}{-0.36\%} \\
   & conjunction &      70.55\% & 71.99\% &    \textcolor{red}{1.44\%} \\
   & copule &      72.28\% & 71.80\% & \textcolor{green}{-0.48\%} \\
   & det &      71.10\% & 72.19\% &    \textcolor{red}{1.09\%} \\
   & mark &      70.87\% & 72.05\% &    \textcolor{red}{1.18\%} \\
   & mwe &      72.39\% & 72.17\% & \textcolor{green}{-0.22\%} \\
   & name &      71.93\% & 72.04\% &    \textcolor{red}{0.11\%} \\
ru & case &      69.86\% & 69.31\% & \textcolor{green}{-0.56\%} \\
   & conjunction &      68.85\% & 69.37\% &    \textcolor{red}{0.51\%} \\
   & copule &      69.49\% & 69.54\% &                     0.06\% \\
   & det &      69.52\% & 69.26\% & \textcolor{green}{-0.25\%} \\
   & mark &      69.04\% & 69.54\% &    \textcolor{red}{0.50\%} \\
   & mwe &      69.41\% & 69.13\% & \textcolor{green}{-0.28\%} \\
   & name &      69.31\% & 69.10\% & \textcolor{green}{-0.21\%} \\
sl & case &      75.60\% & 75.80\% &    \textcolor{red}{0.21\%} \\
   & conjunction &      74.98\% & 76.05\% &    \textcolor{red}{1.08\%} \\
   & copule &      79.69\% & 76.75\% & \textcolor{green}{-2.95\%} \\
   & det &      75.73\% & 75.75\% &                     0.02\% \\
   & mark &      76.12\% & 75.62\% & \textcolor{green}{-0.50\%} \\
   & mwe &      75.76\% & 75.80\% &                     0.04\% \\
   & name &      75.91\% & 75.88\% &                    -0.03\% \\
sv & case &      77.45\% & 77.34\% & \textcolor{green}{-0.11\%} \\
   & conjunction &      76.77\% & 78.18\% &    \textcolor{red}{1.41\%} \\
   & copule &      79.05\% & 77.96\% & \textcolor{green}{-1.09\%} \\
   & det &      75.43\% & 77.16\% &    \textcolor{red}{1.73\%} \\
   & mark &      76.91\% & 77.34\% &    \textcolor{red}{0.44\%} \\
   & mwe &      77.35\% & 77.22\% & \textcolor{green}{-0.13\%} \\
   & name &      77.22\% & 77.41\% &    \textcolor{red}{0.19\%} \\
ta & case &      70.31\% & 70.37\% &                     0.06\% \\
   & conjunction &      70.02\% & 69.90\% & \textcolor{green}{-0.12\%} \\
   & det &      69.96\% & 70.13\% &    \textcolor{red}{0.18\%} \\
   & mark &      70.77\% & 70.08\% & \textcolor{green}{-0.70\%} \\
tr & case &      67.21\% & 67.11\% &                    -0.10\% \\
   & conjunction &      66.67\% & 67.21\% &    \textcolor{red}{0.53\%} \\
   & copule &      67.09\% & 66.65\% & \textcolor{green}{-0.43\%} \\
   & det &      65.77\% & 67.52\% &    \textcolor{red}{1.75\%} \\
   & mark &      67.11\% & 67.39\% &    \textcolor{red}{0.28\%} \\
zh & case &      68.95\% & 69.36\% &    \textcolor{red}{0.42\%} \\
   & conjunction &      69.20\% & 69.77\% &    \textcolor{red}{0.57\%} \\
   & copule &      69.34\% & 69.51\% &    \textcolor{red}{0.17\%} \\
   & det &      68.30\% & 69.56\% &    \textcolor{red}{1.26\%} \\
   & mark &      66.67\% & 69.65\% &    \textcolor{red}{2.98\%} \\
\end{supertabular}

